Set-Valued Rigid Body Dynamics for Simultaneous, Inelastic, Frictional Impacts

Robotic manipulation and locomotion often entail nearly-simultaneous collisions -- such as heel and toe strikes during a foot step -- with outcomes that are extremely sensitive to the order in which impacts occur. Robotic simulators commonly lack the accuracy to predict this ordering, and instead pick one with a heuristic. This discrepancy degrades performance when model-based controllers and policies learned in simulation are placed on a real robot. We reconcile this issue with a set-valued rigid-body model which generates a broad set of physically reasonable outcomes of simultaneous frictional impacts. We first extend Routh's impact model to multiple impacts by reformulating it as a differential inclusion (DI), and show that any solution will resolve all impacts in finite time. By considering time as a state, we embed this model into another DI which captures the continuous-time evolution of rigid body dynamics, and guarantee existence of solutions. We finally cast simulation of simultaneous impacts as a linear complementarity problem (LCP), and develop an algorithm for tight approximation of the post-impact velocity set with probabilistic guarantees. We demonstrate our approach on several examples drawn from manipulation and legged locomotion.

==> termination.tex <==
\label{section:termination}
While solutions to the underlying differential inclusion are guaranteed to exist in the simultaneous impact model, we have yet to prove that they terminate, as in Routh's single-contact method. Termination proofs for other simultaneous impact models (e.g. \cite{Anitescu97, Drumwright2010, Seghete2014} and others) exist, but these approaches rely on comparatively limited impulsive behaviors, and thus cannot capture essential non-unique post-impact velocities. We now show that our model exhibits what we understand to be the most permissive guaranteed termination behavior:
\begin{theorem}\label{thm:nondegeneratedissipation}
	For any pre-impact velocity $\Velocity(0)$ for a contact set $N \in \NondegenerateContactSystems$, The differential inclusion (\ref{eq:multicontact}) will resolve the impact by some $S$ proportional to $\TwoNorm{\Velocity(0)}$.
\end{theorem}

We will prove this claim as a consequence of kinetic energy decreasing fast enough to force termination---a significant expansion of Theorem \ref{thm:strictdissipation}. Even though $\KineticEnergy$ must always decrease, Theorem \ref{thm:strictdissipation} does not forbid $\TotalDiff{}{s}\KineticEnergy(\Velocity) \StrongConvergence 0$. In fact, it is not possible to create an instantaneous bound $\TotalDiff{}{s}\KineticEnergy(\Velocity) \leq -\epsilon < 0$. For example, consider 2 frictionless, axis-aligned contacts $C$ such that $\J[C] = \Identity_2$. For every $\epsilon > 0$, we can pick a velocity
	\begin{equation}
		\Velocity_\epsilon = (1+\epsilon)\begin{bmatrix}
			-1 \\
			-\epsilon
		\end{bmatrix} \in \ActiveSet[C]\,,
	\end{equation}
	\begin{equation}
		\dot \Velocity_\epsilon = \J[C]^T\begin{bmatrix}
			\epsilon \\ 1
		\end{bmatrix}\frac{1}{1+\epsilon} = \begin{bmatrix}
			\epsilon \\ 1
		\end{bmatrix}\frac{1}{1+\epsilon} \in \DerivativeMap[C](\Velocity_\epsilon)\,,
	\end{equation}
	and arrive at $\dot K > -2\epsilon$. However as we take $\epsilon \StrongConvergence 0$, $\Velocity_\epsilon$ converges to to boundary of $\ActiveSet[C]$ and thus will only be ably to sustain a small $\dot K$ for a small amount of time before terminating the impact. It remains possible that the \textit{aggregate energy dissipation} over an interval of fixed nonzero length can be bounded away from zero. We establish a rigorous characterization of this quality by defining $\DissipationRate(s)$-dissipativity:

\begin{definition}[$\DissipationRate(s)$-dissipativity]
For a positive definite function $\DissipationRate(s):\Closure \Real^+ \rightarrow [0,1)$, the system $\dot\Velocity \in \DerivativeMap[C](\Velocity)$ is said to be $\boldmath{\DissipationRate}(s)$\textbf{-dissipative} if for all $s > 0$, for all $\Velocity \in \SolutionSet{\DerivativeMap[C]}[[0,s]]$ s.t. $\Velocity\Parentheses{[0,s]} \subseteq \ActiveSet[C]$, if $\TwoNorm{\Velocity(0)} = 1$, $\TwoNorm{v(s)} \leq 1 - \DissipationRate(s)$.
\end{definition}
Denote the collection of contact sets with this property as
\begin{equation}
	\DissipativeContactSystems = \Braces{D \in \ContactSystems : \exists \DissipationRate[D](s), D\text{ is }\DissipationRate[D](s)\text{-dissipative} }\,.
\end{equation}
Intuitively, if $K > 0$ on $\ActiveSet[C]$ and $K$ decreases at a known nonzero rate, we can show that any trajectory $\Velocity(s)$ of the multi-contact system will exit $\ActiveSet[C]$ at a time linearly bounded in $\TwoNorm{\Velocity(0)}$:
\begin{lemma}[Bounded Exit]\label{lem:exit}
	Let $\DissipationRate[C](s):\Closure \Real^+ \rightarrow [0,1)$ be positive definite and let $C \in \ContactSystems$ be $\DissipationRate[C](s)$-dissipative. Then $\forall S > 0$, $\forall \Velocity(s) \in \SolutionSet{\DerivativeMap[C]}[\Brackets{0,\TwoNorm{\Velocity(0)}\frac{S}{\DissipationRate[C](S)}}]$, $\Velocity \Parentheses{\Brackets{0,\TwoNorm{\Velocity(0)}\frac{S}{\DissipationRate[C](S)}}} \not \subseteq \ActiveSet[C]$.
\end{lemma}
\begin{proof}
	See Appendix \ref{adx:exitproof}. 
\end{proof}
Any contact set $C$ that complies with the strong assumption of $\DissipationRate(s)$-dissipativity is an element of $\NondegenerateContactSystems$, as otherwise $\Velocity$ and $K$ could be constant (i.e. $\DissipativeContactSystems \subseteq \NondegenerateContactSystems$).
Far more useful is that we will show Theorem \ref{thm:nondegeneratedissipation} arises from the converse: that \textit{every} $C \in \NondegenerateContactSystems$ exhibits $\DissipationRate(s)$-dissipativity. This is particularly surprising for systems $C$ with $\J[C]$ not full rank, as $\Velocity(0)$ could be large, yet $\Velocity_R(s)$, the projection of $\Velocity(s)$ onto $\RangeSpace{\J[C]^T}$, could be arbitrary small, permitting small $\dot K$. We observe that the rank of $\J[C]$ does not effect whether or not $C \in \DissipativeContactSystems$, as all solutions will fall into two categories: either $\Velocity_R(s)$ is large, or the related minimal coordinate system will exit $\ActiveSet[C]$ very quickly:
\begin{theorem}\label{thm:minimalsufficiency}
	$\forall m > 0,m \geq k \geq 0$, $\NondegenerateContactSystems \cap \MinimalContactSystems{m}{k} \subseteq \DissipativeContactSystems \implies \NondegenerateContactSystems \cap \SizedContactSystems{m}{k} \subseteq \DissipativeContactSystems$
\end{theorem}
\begin{proof}
	See Appendix \ref{adx:minimalsufficiency}.
\end{proof}
Finally, we prove the primary claim of this work. Intuitively, if there exists $C \in \NondegenerateContactSystems$ that is not $\DissipationRate(s)$-dissipative, then one could construct a sequence of convergent solutions to $\dot \Velocity \in \DerivativeMap[C]$ that dissipate arbitrarily small amounts of energy. Therefore their limit, also a solution to $\dot \Velocity \in \DerivativeMap[C]$ as the solution set is closed, dissipates no energy---leading to a contradiction with Theorem \ref{thm:strictdissipation}. This argument will be used in an inductive manner, incrementing the size of the contact sets:
\begin{theorem}[Dissipation Inductive Step]\label{thm:incrementaldissipation}
	Assume $\NondegenerateContactSystems \cap \SizedContactSystems{m'}{k'} \subseteq \DissipativeContactSystems$ for all $m' \geq k' \geq 0$ with $k' < k$ or $k'=k$ and $m' < m$. Then $\NondegenerateContactSystems \cap \SizedContactSystems{m}{k} \subseteq \DissipativeContactSystems$.
\end{theorem}
\begin{proof}
	Suppose not. Then by Theorem \ref{thm:minimalsufficiency}, there is a set of contacts $C \in \NondegenerateContactSystems \cap \MinimalContactSystems{m}{k}$, $S > 0$, and a corresponding sequence of solutions $\Parentheses{\Velocity^j(s)}_{j \in \Natural}$, $\Velocity^j(s) \in \SolutionSet{\DerivativeMap[C]}[[0,S]]$, all starting with velocity magnitude $1$ ($\TwoNorm{\Velocity^j(0)} = 1$) and never exiting $\ActiveSet[C]$.
	We must also have that each dissipates less energy than the last: $\TwoNorm{\Velocity^j(s)} > 1 - \frac{1}{j}$. As $\DerivativeMap[C]$ is uniformly bounded, $\Velocity^j$ are unformly bounded and equicontinuous.
	By Theorem \ref{thm:Rellich} and Lemma \ref{lem:NonEmptyClosure}, we may assume that $\exists \Velocity^\infty(s) \in \SolutionSet{\DerivativeMap[C]}[[0,S]]$ such that $\Velocity^j \UniformConvergence \Velocity^\infty$. Therefore $\TwoNorm{\Velocity^\infty(s)} = 1$ for all $s$ and by Theorem \ref{thm:stop} $\Velocity^\infty$ is constant. As $C \in \NondegenerateContactSystems$, by Theorem \ref{thm:strictdissipation}, $\Velocity^\infty$ is not an element of $\ActiveSet[C]$ (i.e., $\Jn[C] \Velocity^\infty \geq \ZeroVector$). As $\J[C]$ is full rank, $\J[C] \Velocity^\infty \neq \ZeroVector$. Let $\Force[C]^j(s)$ be the corresponding force vector for each $\Velocity^j(s)$.
	
		Case 1: One contact has strictly deactivated ($\exists c \in C$, $\Jn[c] \Velocity^\infty > \ZeroVector$). But then as $\Velocity^j \UniformConvergence \Velocity^\infty$, by taking a subsequence starting from sufficiently high $j$ we may assume that $c$ \textit{never} activates ($\forall j,t,\Jn[c] \Velocity^j(s) > \ZeroVector$), and therefore at least one of the other contacts is always active ($\Velocity^j([0,S]) \subseteq \ActiveSet[C \setminus \Braces{c}]$). But then only the forces from $C \setminus \Braces{c}$ determine $\dot \Velocity^j$, and thus $\Velocity^j \in \SolutionSet{\DerivativeMap[C \setminus \Braces{c}]}[[0,S]]$. As removing a contact shrinks the set of possible forces to apply ($\NetForce[C \setminus \{c\}] \subseteq \NetForce[C]$), $C \setminus \Braces{c} \in \NondegenerateContactSystems$ and contains $m-1$ contacts. Then by assumption, for some $\DissipationRate(s)$, $C \setminus \Braces{c}$ is $\DissipationRate(s)$-dissipative. But $\TwoNorm{\Velocity^j(s)} \StrongConvergence 1$. Contradiction!
		\begin{figure}[h]
		\vspace{0.5mm}
		\centering
			\includegraphics[width=.50\hsize]{ConvexContactCombination}
			\caption{Conversion of a frictional contact into three frictionless contacts. As $j \StrongConvergence \infty$, we can contain $\FrictionForce[w]^j$ in an arbitrarily small neighborhood around $-\FrictionCoeff[w]\NormalForce[w]^j\Direction{\Jt[w]\Velocity^\infty}$. We pick the neighborhood to be a small triangle with vertices $\vect d_{i,w}$, such that all $\FrictionForce[w]^j$ lie in $\NormalForce[w]\Hull\Parentheses{\Braces{\vect d_{1,w},\vect d_{2,w},\vect d_{3,w}}}$, thus (\ref{eq:contactcomposition}). If the triangle is small, each $\vect d_i$ will be nearly anti-parallel to $\Jt[w]\Velocity^\infty$, implying (\ref{eq:persistence}).}
			\label{fig:contactconversion}
			
		\end{figure}
		
		Case 2: At least one contact always slides $\Parentheses{\Jt[C]\Velocity^\infty \neq \ZeroVector,\,\Jn[C]\Velocity^\infty = \ZeroVector}$.
		Let $W = \Braces{ w \in C :\TwoNorm{\Jt[w] \Velocity^\infty} > \ZeroVector} \neq \emptyset$ be the set of contacts that slide for velocity $\Velocity^\infty$.
		Then as $\Unit$ is u.s.c., $\forall w \in W,\, \Unit\Parentheses{\Jt[w] \Velocity^j} \UniformConvergence \Unit\Parentheses{\Jt[w] \Velocity^\infty}$ (i.e. convergence of the velocity to $\Velocity^\infty$ implies convergence of the direction of sliding on each contact in $W$).
		Therefore WLOG by taking a subsequence starting from sufficiently high $j$ we may assume $\forall w \in W,\, \exists \vect d_{1,w},\vect d_{2,w},\vect d_{3,w}$ sufficiently close to $-\FrictionCoeff[w]\Direction{\Jt[w] \Velocity^\infty}$ and associated new contacts $\bar w_1, \bar w_2, \bar w_3$ such that
		\begin{align}
			\Jn[\bar w_i] &= \Jn[w] + \vect d_{i,w}^T \Jt[w],\\
			\Jn[\bar w_i] \Velocity^j (s) &< 0,\label{eq:persistence} \\
			\J[w]^T\Force[w]^j (s) &\in \NormalForce[w]^j(s)\Hull\Parentheses{\bigcup_i\Braces{\Jn[\bar w_i]}} a.e.\,,\label{eq:contactcomposition}
		\end{align}
		for $i \in \Braces{1,2,3}$.
		Denote $\bar W = \bigcup_{i,w} \bar w_i$ and $\bar C = (C \cup \bar W)\setminus W$.
		(\ref{eq:persistence}) and (\ref{eq:contactcomposition}) in conjunction imply that, for velocities $\Velocity^j (s) \approx \Velocity^\infty$, each sliding frictional contact pushes mostly in one direction.
		Furthermore, the associated frictional force can be generated by three frictionless contacts tilted away from the sliding direction ($\Velocity^j \in \SolutionSet{\DerivativeMap[\bar C]}[[0,S]]$) which never deactivate ($\Velocity^j([0,S]) \subseteq \ActiveSet[\bar C]$). Figure \ref{fig:contactconversion} illustrates this construction.
		As $\bar C$ has strictly fewer frictional contacts than $C$ and is not $\DissipationRate(s)$-dissipative ($\TwoNorm{\Velocity^j(s)} \StrongConvergence 1$), by assumption we must have that $\bar C \not \in \NondegenerateContactSystems$.
		By definition of $\NondegenerateContactSystems$ there must exist some penetrating velocity $\Velocity \in \ActiveSet[\bar C]$ such that $\ZeroVector \in \NetForce[\bar C](\Velocity)$ is a permissible net force.
		We therefore must be able to find individual contact forces $\NormalForce[\bar c]f_{\bar c}$ with $\NormalForce[\bar c] \geq 0$ and $f_{\bar c} \in \NetForce[\bar c]\Parentheses{\Velocity}$ for each contact $\bar c \in \bar C$ such that $\sum_{\bar c \in \bar C} \NormalForce[\bar C] = 1$ and $\sum_{\bar c \in \bar C} \NormalForce[\bar c]f_{\bar c} = \ZeroVector$.
		As no combination of the original contacts $C$ can create zero net force alone, one of the $\bar w \in \bar W$ must strictly activate ($\NormalForce[\bar w]f_{\bar w} \neq 0$). By construction of $W$ and $\bar W$ and the assumption of Case 2, we have $\J[ C \setminus W]\Velocity^\infty = \ZeroVector$, and thus $f_{\bar c}^T\Velocity^\infty = 0$ for each $\bar c \in C \setminus W$ and $f_{\bar w}^T\Velocity^\infty < 0$ for each $\bar w \in \bar W$. Thus $\sum_{\bar c \in \bar C} \NormalForce[\bar c]f_{\bar c}^T \Velocity^\infty < 0$. But then $\sum_{\bar c \in \bar C} \NormalForce[\bar c]f_{\bar c} \neq \ZeroVector$. Contradiction!
		\end{proof}
        We are now ready to prove the main result of this section.
		\begin{proof}[Proof of Theorem \ref{thm:nondegeneratedissipation}] We will reach the claim by showing $\NondegenerateContactSystems = \DissipativeContactSystems$.
		$\NondegenerateContactSystems \supseteq \DissipativeContactSystems$ trivially. Any $C \in \MinimalContactSystems{1}{0}$ is of the form
			\begin{align}
				\DerivativeMap[C](\Velocity) = \begin{cases}
					\Braces\ZeroVector  & \InactiveSet[C] = \{j\Velocity > 0\}\\
					\Braces j & \ActiveSet[C] = \{j\Velocity < 0\} \\
					\Hull \Parentheses{\Braces{0,j}} & j\Velocity = 0
				\end{cases}
			\end{align}
			with $\Velocity, j \in \Real$, $j \neq 0$. Such a system is $\DissipationRate[C]$-dissipative with
			\begin{equation}
				\DissipationRate[C](s) = \min \Braces{\Norm{j}t,\frac{1}{2}}.
			\end{equation}
			$\SizedContactSystems{1}{0} \subseteq \DissipativeContactSystems$ by Theorem \ref{thm:minimalsufficiency}. $\NondegenerateContactSystems \subseteq \DissipativeContactSystems $ follows from nested induction on $(m,k)$ via Theorem \ref{thm:incrementaldissipation}. Therefore, $\NondegenerateContactSystems = \DissipativeContactSystems $.
		\end{proof}

==> verification.tex <==
\label{section:verification}
When $S \in \ContactSystems$ contains a large number of contacts, $S \in \NondegenerateContactSystems$ can be quite difficult to verify by hand; therefore, there is value in creating a numerical algorithm for generating certificates for this condition. To that end, we consider a slightly smaller collection of contact sets

\begin{equation}
	\NondegenerateContactSystems^* = \Braces{N \in \ContactSystems : \ZeroVector \not \in \NetForce[N]\Parentheses{\Closure\ActiveSet[N]} } \subseteq \NondegenerateContactSystems\,.
\end{equation}
For any $N \in \NondegenerateContactSystems^*$, not only is $\ZeroVector \not \in \NetForce[N]\Parentheses{\Closure\ActiveSet[N]}$, but we can find an $\epsilon > 0$ such that $\NetForce[N]\Parentheses{\Closure\ActiveSet[N]}$ is bounded at least $\epsilon$ away from $\ZeroVector$:
\begin{theorem}
	If $N \in \NondegenerateContactSystems^*$, $\exists \epsilon > 0$, $\NetForce[N]\Parentheses{\Closure\ActiveSet[N]} \cap \Ball_\epsilon = \emptyset$. 
\end{theorem}
\begin{proof}
	Suppose not. Then, for some $N \in \NondegenerateContactSystems^*$. $\exists \Sequence{\Velocity}{k}, \Sequence{\dot \Velocity}{k}$, $\Velocity_k \in \Closure\ActiveSet[N]$ and $\dot \Velocity_k \in \NetForce[N]\Parentheses{\Velocity_k}$ for all $k$ and $\dot \Velocity_k \StrongConvergence 0$. WLOG as $\dot \Velocity_k \in \NetForce[S]\Parentheses{\Direction\Velocity_k}$ for $\Velocity_k \neq \ZeroVector$, we may assume that $\Sequence{\Velocity}{k}$ is bounded. As $\Sequence{\Velocity}{k}$ and $\Sequence{\dot \Velocity}{k}$ are bounded, by dropping to a subsequence WLOG we may assume $\exists \Velocity_\infty$, $\Velocity_k \StrongConvergence \Velocity_\infty \in \Closure\ActiveSet[N]$. But then as $\NetForce[S]$ is u.s.c., $\ZeroVector \in \NetForce[S]\Parentheses{\Velocity_\infty}$ and therefore $N \not \in \NondegenerateContactSystems^*$. Contradiction!
\end{proof}
For any $\Velocity \in \Closure\ActiveSet[N], \dot \Velocity \in \NetForce[N](\Velocity)$, we have that $\dot \Velocity = \J[N]^T\Force[N]$ with $\Force[N] \in \FrictionCone[S](\Velocity)$ both bounded and bounded away from $\ZeroVector$; additionally, for any $\Velocity \not \in \Closure\ActiveSet[N]$, we have $\FrictionCone[S](\Velocity) = \{\ZeroVector\}$. Therefore, the condition $N \in \NondegenerateContactSystems^*$ is equivalent to the existence of an $\epsilon > 0$ such that
\begin{equation}
	\Force[N] \in \FrictionCone[S](\Velocity) \implies \TwoNorm{\J[N]\Force[N]}^2 - \epsilon \TwoNorm{\Force[N]}^2 \geq 0\,.\label{eq:semialgnondegenerate}
\end{equation}
We note that (\ref{eq:semialgnondegenerate}) is formatted as non-negativity of the polynomial $\TwoNorm{\J[N]\Force[N]}^2 - \epsilon \TwoNorm{\Force[N]}^2$ on a set $\FrictionCone[S](\Velocity)$ that can defined by polynomial inequalities and equalities \cite{Posa16}. Therefore, a certificate for $N \in \NondegenerateContactSystems^*$ can be generated by a sum-of-squares program that finds the maximal $\epsilon$ for which $N$ obeys (\ref{eq:semialgnondegenerate}).

